Covering arrays from maximal sequences over finite fields

The focus of this thesis is the study and construction of covering arrays, relying on maximal period sequences and other tools from finite fields. A covering array of strength $t$, denoted $\mathrm{CA}(N; t, k,v)$, is an $N\times k$ array with entries from an alphabet $A$ of size $v$, with the property that in the $N\times t$ subarray defined by any $t$ columns, each of the $v^t$ vectors in $A^t$ appears at least once as a row. Covering arrays generalize orthogonal arrays, which are classic combinatorial objects that have been studied extensively. Constructing covering arrays with a small row-to-column ratio is important in the design of statistical experiments, however it is also a challenging mathematical problem. Linear feedback shift register (LFSR) sequences are sequences of elements from a finite field that satisfy a linear recurrence relation. It is well-known that these are periodic; LFSR sequences that attain the maximum possible period are maximal (period) sequences, often abbreviated to m-sequences in the literature. Arrays constructed from cyclic shifts of maximal sequences possess strong combinatorial properties and have been previously used to construct orthogonal and covering arrays (Moura et al., 2016), although only one of the known constructions is for covering arrays that are not orthogonal arrays (Raaphorst et al., 2014). In this thesis we present several new such constructions. The cornerstone of our results is a study of the combinatorial properties of arrays constructed from maximal sequences, where we make fundamental connections with concepts from diverse areas of discrete mathematics, such as orthogonal arrays, error-correcting codes, divisibility of polynomials and structures of finite geometry. One aspect of our work involves [..]

==> ALGORITHMS/Precalculation.tex <==
\begin{algorithm}[t]
    \caption{Precalculation of $U_P$ for use in \Cref{algorithm:ExtendCM}}
    \label{algorithm:Precalculation}
    \begin{algorithmic}%[1]
    \Procedure{Precalculate$U_P$}{$\a_0, \dots, \a_{l-1}$}
    %\algrenewcommand\algorithmicindent{2.0em}%
       \For{$I \in \binom{[1,\w{t}-1]}{t-2}$}
           \State $U(I)\gets \emptyset$
       \EndFor
       \For{$i$ from $0$ to $l-1$}
           \State $z_i \gets \{j \in [0, \w{t}-1]\mid \Tt(\a_i^{j})=0\}$
           \For{$d$ in $z_i$}
               \State $Z\gets \{(j-d) \bmod{\w{t}} \mid j \in z_i \text{ and } j \neq d\}$
               \For{$I \in \binom{Z}{t-2}$}
                   \State $U(I)\gets U(I)\cup (Z\setminus I)$
               \EndFor
           \EndFor
       \EndFor
       \Return $U$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}



==> TABLES/ArrayModVExamples.tex <==
\begin{table}
\[
        \M{\a}=
        \begin{array}{llllllll}
            2&1&2&6&0&3&3&1
        \end{array}
        \quad\quad
        \begin{array}{rllllllll}
            \multirow{8}{*}{$\MV{\a}=$}    
            2&0&2&0&z&1&1\\
            0&2&0&z&1&1&0\\
            2&0&z&1&1&0&0\\
            0&z&1&1&0&0&1\\
            z&1&1&0&0&1&0\\
            1&1&0&0&1&0&1\\
            1&0&0&1&0&1&z\\
            0&0&1&0&1&z&2\\
            0&1&0&1&z&2&2\\
            1&0&1&z&2&2&1\\
            0&1&z&2&2&1&1\\
            1&z&2&2&1&1&2\\
            z&2&2&1&1&2&1\\
            2&2&1&1&2&1&2\\
            2&1&1&2&1&2&z\\
            1&1&2&1&2&z&0\\
            1&2&1&2&z&0&0\\
            2&1&2&z&0&0&2\\
            1&2&z&0&0&2&2\\
            2&z&0&0&2&2&0\\
            z&0&0&2&2&0&2\\
            0&0&2&2&0&2&0\\
            0&2&2&0&2&0&z\\
            2&2&0&2&0&z&1\\
             & & & & & & \\
             & & & & & &
        \end{array}
    \]
    \label{aaa}
    \caption{rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\end{table}


==> TABLES/Experiments2ndPaperStrength3.tex <==
\[
\renewcommand{\arraystretch}{\genarraystretch}
    \rowcolors{2}{\backgroundshade}{white}
    \begin{array}{rlll}
    \rowcolor{\tableheadcolor}
    v
    &\multicolumn{1}{l}{\text{Successful $q$ below theoretical guarantee}}
    &\multicolumn{1}{l}{\text{Values of $q$ tested}}
    &\multicolumn{1}{l}{\text{Theoretical guarantee}}
    \\
    2   & \text{None}                                      &q <    7   & q\geq 7         \\
    3   & \text{None}                                      &q <    19  & q\geq 19        \\
    4   & q\geq 37,  \text{ except } 41                    &q <    61  & q\geq 61        \\
    5   & q\geq 81,  \text{ except } 101                   &q <    181 & q\geq 181       \\
    6   & q\geq 103, \text{ except } 109,139,157,223,277   &q <    439 & q\geq 439       \\
    7   & q \geq 169                                       &q \leq 379 & q\geq 953       \\
    8   & 193,241,281,313                                  &q \leq 337 & q\geq 1849      \\
    9   & 289                                              &q \leq 523 & q\geq 3259      \\
    10  & 361                                              &q \leq 491 & q\geq 5261      \\
    11  & 243,397                                          &q \leq 463 & q\geq 8273      \\
    12  & \text{None}                                      &q \leq 457 & q\geq 12241     
    \end{array}
\]


==> TABLES/SeqVExample.tex <==
\begin{table}[t]
%\renewcommand{\arraystretch}{1.3}
\rowcolors{2}{beach!15}{white}
\[
%\newcolumntype{I}{>{\hfill}>{$}m{3.5em}<{$}}
%\newcolumntype{L}{>{$}p{1.08em}<{$}}
%\begin{array}[]{I|*{18}l}
\begin{array}{llllll}
\rowcolor{beach!70}
\multicolumn{1}{c}{i} & 0     & 1         & 2         & 3         & 4 \\
\Tt(\b^i)        &  \o &\o       &1 &\o &0   \\
\logw(\Tt(\b^i)) & 	1 &1       &0 &1 & -   \\
\seqv{\b}_i      & 	1 &1       &0 & 1 & \mathbf{0}   \\
\rowcolor{beach!70}
 \multicolumn{1}{c}{i} &    	5    &6    &7    &8    &9 \\
\Tt(\b^i)        &  \o+1 &\o+1       &\o &\o+1 &0   \\
\logw(\Tt(\b^i)) & 	2 &2       &1 &2 &-   \\
\seqv{\b}_i      & 	2 &2       &1 &2 &\mathbf{0}   \\
\rowcolor{beach!70}
\multicolumn{1}{c}{i} &10 &11 &12 &13 &14  \\
\Tt(\b^i)        &  1 &1       &\o+1 &1 &0   \\
\logw(\Tt(\b^i)) & 	0 &0       &2 &0 &1   \\
\seqv{\b}_i      & \mathbf{0}	 & \mathbf{0}  & 2 & \mathbf{0} &1
\end{array}
\]
\caption{Demonstration of the sequences in \Cref{example:SeqModVFirstExample}}
\label{table:ExampleSequenceModV}
\end{table}




==> TABLES/SeqVExample1.tex <==
\begin{table}
\[
        \M{\a}=
        \begin{array}{llllllll}
            2&1&2&6&0&3&3&1
        \end{array}
        \quad\quad
        \begin{array}{rllllllll}
            \multirow{8}{*}{$\MV{\a}=$}    
            2&0&2&0&z&1&1\\
            0&2&0&z&1&1&0\\
            2&0&z&1&1&0&0\\
            0&z&1&1&0&0&1\\
            z&1&1&0&0&1&0\\
            1&1&0&0&1&0&1\\
            1&0&0&1&0&1&z\\
            0&0&1&0&1&z&2\\
            0&1&0&1&z&2&2\\
            1&0&1&z&2&2&1\\
            0&1&z&2&2&1&1\\
            1&z&2&2&1&1&2\\
            z&2&2&1&1&2&1\\
            2&2&1&1&2&1&2\\
            2&1&1&2&1&2&z\\
            1&1&2&1&2&z&0\\
            1&2&1&2&z&0&0\\
            2&1&2&z&0&0&2\\
            1&2&z&0&0&2&2\\
            2&z&0&0&2&2&0\\
            z&0&0&2&2&0&2\\
            0&0&2&2&0&2&0\\
            0&2&2&0&2&0&z\\
            2&2&0&2&0&z&1\\
             & & & & & & \\
             & & & & & &
        \end{array}
    \]
    \label{aaa}
    \caption{rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\end{table}


==> TABLES/SeqVExample2.tex <==
\begin{table}[t]
%\rowcolors{2}{beach!15}{white}
%\renewcommand{\arraystretch}{1.3}
\rowcolors{2}{beach!15}{white}
\[
    \begin{array}{*{9}l}
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
        \seq{\a}_i & 2& 1& 2& 6& 0& 3& 3& 1\\
        \logw(\seq{\a}_i) & 2& 0& 2& 3& -& 1& 1& 0\\
        \seqv{\a}_i & 2& 0& 2& 0& \mathbf{0}& 1& 1& 0\\
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\
        \seq{\a}_i & 6& 3& 6& 4& 0& 2& 2& 3\\
        \logw(\seq{\a}_i) & 3& 1& 3& 4& -& 2& 2& 1\\
        \seqv{\a}_i & 0& 1& 0& 1& \mathbf{0}& 2& 2& 1\\
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 \\
        \seq{\a}_i & 4& 2& 4& 5& 0& 6& 6& 2\\
        \logw(\seq{\a}_i) & 4& 2& 4& 5& -& 3& 3& 2\\
        \seqv{\a}_i & 1& 2& 1& 2& \mathbf{0}& 0& 0& 2\\
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 \\
        \seq{\a}_i & 5& 6& 5& 1& 0& 4& 4& 6\\
        \logw(\seq{\a}_i) & 5& 3& 5& 0& -& 4& 4& 3\\
        \seqv{\a}_i & 2& 0& 2& 0& \mathbf{0}& 1& 1& 0\\
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 \\
        \seq{\a}_i & 1& 4& 1& 3& 0& 5& 5& 4\\
        \logw(\seq{\a}_i) & 0& 4& 0& 1& -& 5& 5& 4\\
        \seqv{\a}_i & 0& 1& 0& 1& \mathbf{0}& 2& 2& 1\\
\rowcolor{beach!70}
        \multicolumn{1}{c}{i} & 40 & 41 & 42 & 43 & 44 & 45 & 46 & 47\\
        \seq{\a}_i & 3& 5& 3& 2& 0& 1& 1& 5\\
        \logw(\seq{\a}_i) & 1& 5& 1& 2& -& 0& 0& 5\\
        \seqv{\a}_i & 1& 2& 1& 2& \mathbf{0}& 0& 0& 2
    \end{array}
\]
\caption{Demonstration of the sequences in \Cref{example:SeqModVSecondExample}}
\label{table:ExampleSequenceModV2}
\end{table}





==> _Theorem_environments.tex <==
\def\myskip{10pt}
\tcbset{
%%%%% Starting tcbset %%%%%
theostyle/.style={
%%%%breakable,
%%%%enhanced,
%%%%fonttitle=\bfseries\upshape,
%%%%fontupper=\slshape,
%%%% before skip=\baselineskip,
%%%%arc=0.8mm,  coltitle=black,colbacktitle=pond, colback=beach!30, colframe=pond,boxrule=0.4mm,
%%%%attach boxed title to top left={xshift=1cm,yshift*=1mm-\tcboxedtitleheight},
%%%%varwidth boxed title*=-3cm,
%%%%boxed title style={frame code={
%%%%\path[fill=tcbcol@back!50!black]
%%%%([yshift=-1mm,xshift=-1mm]frame.north west)
%%%%arc[start angle=0,end angle=180,radius=1mm]
%%%%([yshift=-1mm,xshift=1mm]frame.north east)
%%%%arc[start angle=180,end angle=0,radius=1mm];
%%%%\path[left color=tcbcol@back,right color=tcbcol@back,
%%%%middle color=tcbcol@back!60!beach]
%%%%([xshift=-2mm]frame.north west) -- ([xshift=2mm]frame.north east)
%%%%[rounded corners=1mm]-- ([xshift=1mm,yshift=-1mm]frame.north east)
%%%%-- (frame.south east) -- (frame.south west)
%%%%-- ([xshift=-1mm,yshift=-1mm]frame.north west)
%%%%[sharp corners]-- cycle;
%%%%},interior engine=empty,
%%%%},
%%%%fonttitle=\bfseries,
%%%%description delimiters none,% parenthesis,
%%%%separator sign= {:},
%%%%terminator sign={.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    theorem style=plain,
    fonttitle=\bfseries\upshape,
    fontupper=\slshape,
    breakable,
    enhanced,
    arc=0.2mm, 
    boxrule=0.3mm, 
    colback=\backgroundshade,
    colframe=\theocolor,
    coltitle=black,
    description delimiters parenthesis,
    separator sign= {},
    terminator sign={.},
    borderline west={2mm}{0mm}{\theocolor}
},
plaintheostyle/.style={
    theorem style=plain,
    fonttitle=\bfseries\upshape,
    fontupper=\slshape,
    breakable,
    enhanced,
    arc=0.2mm, 
    boxrule=0.3mm, 
%    before skip=\baselineskip,
%    top=0mm,
%    bottom=0mm,
%    left=0mm,
%    right=0mm,
    colback=\backgroundshade,
    colframe=\generaltheocolor,
    coltitle=black,
    description delimiters parenthesis,
    separator sign= {},
    terminator sign={.},
    borderline west={2mm}{0mm}{\generaltheocolor}
},
defstyle/.style={
%%%%breakable,
%%%%enhanced,
%%%% before skip=\baselineskip,
%%%%fonttitle=\bfseries\upshape,
%%%%fontupper=\upshape,%\slshape,
%%%%arc=0.8mm,  coltitle=black,colbacktitle=goldfish!70!white, colback=beach!30, colframe=goldfish,boxrule=0.4mm,
%%%%attach boxed title to top left={xshift=1cm,yshift*=1mm-\tcboxedtitleheight},
%%%%varwidth boxed title*=-3cm,
%%%%boxed title style={frame code={
%%%%\path[fill=tcbcol@back!70!black]
%%%%([yshift=-1mm,xshift=-1mm]frame.north west)
%%%%arc[start angle=0,end angle=180,radius=1mm]
%%%%([yshift=-1mm,xshift=1mm]frame.north east)
%%%%arc[start angle=180,end angle=0,radius=1mm];
%%%%\path[left color=tcbcol@back,right color=tcbcol@back,
%%%%middle color=tcbcol@back!60!beach]
%%%%([xshift=-2mm]frame.north west) -- ([xshift=2mm]frame.north east)
%%%%[rounded corners=1mm]-- ([xshift=1mm,yshift=-1mm]frame.north east)
%%%%-- (frame.south east) -- (frame.south west)
%%%%-- ([xshift=-1mm,yshift=-1mm]frame.north west)
%%%%[sharp corners]-- cycle;
%%%%},interior engine=empty,
%%%%},
%%%%fonttitle=\bfseries,
%%%%description delimiters parenthesis,
%%%%separator sign= {},
%%%%terminator sign={.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    theorem style=plain,
    fonttitle=\bfseries\upshape,
    fontupper=\upshape,
    breakable,
    enhanced,
    arc=0.2mm, 
    boxrule=0.3mm, 
    colback=\backgroundshade,
    colframe=\defcolor,
    coltitle=black,
    description delimiters parenthesis,
    separator sign= {},
    terminator sign={.},
    borderline west={2mm}{0mm}{\defcolor}
    }
%%%%% Finishing tcbset %%%%%
}

\newtcbtheorem[number within=chapter,crefname={theorem}{theorems}]%
{theorem} % \begin..
{Theorem} % Title
{theostyle}
{theorem} % label prefix; cite as ``theo:yourlabel''

\newtcbtheorem[use counter from=theorem,crefname={definition}{definitions}]%
{definition} % \begin..
{Definition} % Title
{defstyle} % Style
{definition} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={lemma}{lemmas}]%
{lemma} % \begin..
{Lemma} % Title
{plaintheostyle} % Style
{lemma} % label prefix

\newtcbtheorem[crefname={problem}{problems}]%
{problem} % \begin..
{Problem} % Title
{plaintheostyle} % Style
{problem} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={question}{questions}]%
{question} % \begin..
{Question} % Title
{plaintheostyle} % Style
{question} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={method}{Method}]%
{method} % \begin..
{Method} % Title
{plaintheostyle} % Style
{method} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={proposition}{propositions}]%
{proposition} % \begin..
{Proposition} % Title
{plaintheostyle} % Style
{proposition} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={corollary}{corollaries}]%
{corollary} % \begin..
{Corollary} % Title
{plaintheostyle} % Style
{corollary} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={remark}{remarks}]%
{remark} % \begin..
{Remark} % Title
{   
%    theorem style=margin,
    theorem style=plain,
    label type=remark,
    fonttitle=\slshape,
    fontupper=\upshape,
    breakable,
%    before skip=\baselineskip,
%    after skip=\baselineskip,
    arc=0.2mm, 
    boxrule=0mm, 
    top=0mm,
    bottom=0mm,
    left=0mm,
    right=0mm,
    colback=white,
%    colframe=pond!50!black,
    coltitle=black,
    colframe=white,
    boxsep=0pt, % Otherwise there is slight right shift of the text
%    description delimiters parenthesis,
%    separator sign none,
    terminator sign={.}
} % Style
{remark} % label prefix

\newtcbtheorem[use counter from=theorem,crefname={example}{examples}]%
{example} % \begin..
{Example} % Title
{  theorem style=plain,
%    before skip=\baselineskip,
   colback=white,%beach!20,
   breakable,
   enhanced,
   fonttitle=\Large,
   description font=\normalsize\upshape,
   coltitle=\excolor!10!black,
   parbox=false, % To fix indentation
   boxrule=0.3mm, 
   arc=0.2mm, 
   colframe=\excolor,
   borderline west={2mm}{0mm}{\excolor},
   terminator sign={.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%empty,
%%breakable,
%%coltitle=aoi!15!black,
%%fonttitle=\bfseries,
%%%borderline horizontal={0.5mm}{0pt}{aoi!50!white},
%%borderline={0.5mm}{0pt}{aoi!50!white},
%%titlerule style={aoi}, %arrows = {Hooks[arc=270]-Hooks[arc=270]}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
{example} % label prefix

\tcolorboxenvironment{proof}{% ’proof’ from ’amsthm’
blanker,
breakable,
parbox=false % To fix indentation
%    before skip=\baselineskip,
%enhanced,
%boxrule=0pt,
%rame hidden,
%borderline north={1mm}{-2mm}{red},
%borderline south={1mm}{-2mm}{blue},
%borderline west={2mm}{-2mm}{\proofbordercolor},
%borderline south={2mm}{-2mm}{\proofbordercolor}
}

%\tcolorboxenvironment{algorithmic}{% ’proof’ from ’amsthm’
%%blanker,
%%breakable,
%%parbox=false % To fix indentation
%%    before skip=\baselineskip,
%%enhanced,
%%boxrule=0pt,
%%rame hidden,
%%borderline south={1mm}{-2mm}{blue},
%%borderline west={2mm}{-2mm}{\proofbordercolor},
%%borderline south={2mm}{-2mm}{\proofbordercolor}
%blanker,
%fontupper=\upshape,
%enhanced,
%%arc=0.2mm, 
%boxrule=0mm, 
%colback=white,
%colframe=white,
%coltitle=black,
%borderline west={2mm}{0mm}{black!50}
%}

\def\myqedsymbol{
\tikz\filldraw [ fill=beach, draw=black!20!beach,
line width=0.1mm ] (0,0) rectangle +(0.23,0.23);
}

\renewcommand{\qedsymbol}{\myqedsymbol}


